LinearPartition: Linear-Time Approximation of RNA Folding Partition Function and Base Pairing Probabilities

RNA secondary structure prediction is widely used to understand RNA function. Recently, there has been a shift away from the classical minimum free energy (MFE) methods to partition function-based methods that account for folding ensembles and can therefore estimate structure and base pair probabilities. However, the classical partition function algorithm scales cubically with sequence length, and is therefore a slow calculation for long sequences. This slowness is even more severe than cubic-time MFE-based methods due to a larger constant factor in runtime. Inspired by the success of our recently proposed LinearFold algorithm that predicts the approximate MFE structure in linear time, we design a similar linear-time heuristic algorithm, LinearPartition, to approximate the partition function and base pairing probabilities, which is shown to be orders of magnitude faster than Vienna RNAfold and CONTRAfold (e.g., 2.5 days vs. 1.3 minutes on a sequence with length 32,753 nt). More interestingly, the resulting base pairing probabilities are even better correlated with the ground truth structures. LinearPartition also leads to a small accuracy improvement when used for downstream structure prediction on families with the longest length sequences (16S and 23S rRNA), as well as a substantial improvement on long-distance base pairs (500+ nt apart).

==> fig_correlation.tex <==
\begin{figure*}%[!h]
\center
% \begin{tabular}{c|c|c|c}
\definecolor{darkgreen}{rgb}{0, 0.5, 0}
\newcommand{\bluetri}{{\color{blue} $\blacktriangle$}}
\newcommand{\greentri}{{\color{darkgreen} $\blacktriangle$}}
\newcommand{\redtri}{{\color{red} $\blacktriangle$}}
\newcommand{\bluecir}{{\color{blue} $\circ$}}
\newcommand{\greencir}{{\color{darkgreen} $\circ$}}
\newcommand{\redcir}{{\color{red} $\circ$}}
\begin{tabular}{ccc}
\hspace{-7cm}\panel{A} & \hspace{-2cm}\panel{C} & \hspace{-3.5cm}\panel{D}\\[-1cm]
\raisebox{10.7cm}{\hspace{-0.2cm}\includegraphics[width=0.4\textwidth]{figs/ensemble_defect}} &
% \hspace{-.2cm}\panel{A} & \hspace{-0.6cm}\panel{B} \\[-1cm] %& \hspace{-2.5cm}\panel{D}
	\multicolumn{2}{c}{
	  \hspace{-.7cm}
	  \raisebox{12.4cm}{\includegraphics[width=5.2cm]{figs/prob_xy_grp1}}
	  \hspace{-5.1cm}
	  \raisebox{4cm}{\includegraphics[width=0.58\textwidth]{figs/grp1_70_gutell_modified_2020}}
  	} \\[-11cm]
\hspace{-7cm}\panel{B} &\\[-.5cm]
\raisebox{.cm}{\hspace{-0.2cm}\includegraphics[width=0.42\textwidth]{figs/ensemble_defect_histogram}} & \\[-.4cm]
% \hspace{-.2cm}\raisebox{1cm}{\panel{C}} & \\[-1cm]
\hspace{-7cm}\panel{E} &\\[-.5cm]
\multicolumn{2}{l}{% \hspace{-0.3cm}
\resizebox{0.58\textwidth}{!}{
  \begin{tabular}{cr@{\; }r@{\quad \quad}r@{\; }r}
%	\toprule
         &     \multicolumn{2}{c}{total} & \multicolumn{2}{c}{correct} \\
			 \midrule
{\color{blue} $p_\linear \!-\! p_\vienna \!>\! 0.2$} & 55 \bluetri & 40 \bluecir  & 23 \bluetri & 37 \bluecir \\
{\color{darkgreen} $|p_\linear \!-\! p_\vienna| \!\leq \!0.2$} &  126,645 \greentri & 420 \greencir & 111 \greentri & 180 \greencir\\
{\color{red} $p_\linear \!-\! p_\vienna \!<\! -0.2$} & 56 \redtri & 44 \redcir & 0 \redtri & 19 \redcir \\[1.9cm]
%	                 \bottomrule
  \end{tabular}}
}
\end{tabular}\\[-2cm]
\begin{tabular}{cccc}
\hspace{-4.4cm} \panel{F} & \hspace{-4.6cm}\panel{G} & \hspace{-4.6cm}\panel{H} & \hspace{-4.6cm}\panel{I}\\[-0.2cm]
\hspace{-0.2cm}\includegraphics[width=0.25\textwidth]{figs/23s_gold} &
\hspace{-0.35cm}\includegraphics[width=0.25\textwidth]{figs/23s_vienna_plfold_example.pdf} &
\hspace{-0.35cm}\includegraphics[width=0.25\textwidth]{figs/23s_vienna_example} &
\hspace{-0.35cm}\includegraphics[width=0.25\textwidth]{figs/23s_example.pdf}
\end{tabular}
\caption{
{\bf A}: Ensemble defect comparison between \viennarnafold and \linearpartition on the ArchiveII dataset.
{\bf B}: Ensemble defect difference for each family.
{\bf C--E}: An example of {\it C.~ellipsoidea} Group I Intron. 
{\bf C}: solid triangles ({\small {\color{blue} $\blacktriangle$} {\color{darkgreen}$\blacktriangle$}  {\color{red}$\blacktriangle$}}) stand for base pairing probabilities and
unfilled circles ({\small {\color{blue} $\circ$} {\color{darkgreen}$\circ$}  {\color{red}$\circ$}})  stand for single-stranded probabilities.
{\color{blue} blue: $p_\linear \!-\! p_\vienna \!>\! 0.2$};
{\color{darkgreen} green: $|p_\linear \!-\! p_\vienna| \!\leq \!0.2$};
{\color{red} red: $p_\linear \!-\! p_\vienna \!<\! -0.2$};
%some high probability pairs and unpaired bases in \linearpartition have low probabilities in \viennarnafold (in blue), and some low probability ones in \linearpartition have high probabilities in \viennarnafold (in red); 
	{\bf D}: ground truth structure colored with the above scheme; % from \viennarnafold and \linearpartition; 
	%pink binds around position 370 are pseudoknotted pairs.
	{\bf E}: statistics of this example. 
	"total" columns are the total numbers of triangles and circles with different colors in {\bf A},
	while "correct" columns are the corresponding numbers %of such triangles and circles
        in the ground-truth structure  in {\bf B},
        which is better correlated with \linearpartition's probabilities than \viennarnafold's ({\color{blue} 23 blue pairs} and {\color{red} 0 red pairs}). %ground-truth structure.
	% Note that each triangle represents a pair of nucleotides.
{\bf F--I}: An example of \ecoli 23S rRNA. 
	{\bf F}: circular plot of the ground truth.
{\bf G-I}: circular plots using the base pair probabilities from \viennarnaplfold (with default window size $70$), \rnafold and \linearpartition, respectively; 
base pairs in the ground truth are in blue;
the color shade of the lines are propotional to their probabilities.
	\label{example}\\[-.7cm]
}
\end{figure*}

